Group Buying Recommendation Model Based on Multi-task Learning

In recent years, group buying has become one popular kind of online shopping activity, thanks to its larger sales and lower unit price. Unfortunately, research seldom focuses on recommendations specifically for group buying by now. Although some recommendation models have been proposed for group recommendation, they can not be directly used to achieve real-world group buying recommendation, due to the essential difference between group recommendation and group buying recommendation. In this paper, we first formalize the task of group buying recommendations into two sub-tasks. Then, based on our insights into the correlations and interactions between the two sub-tasks, we propose a novel recommendation model for group buying, MGBR, built mainly with a multi-task learning module. To improve recommendation performance further, we devise some collaborative expert networks and adjusted gates in the multi-task learning module, to promote the information interaction between the two sub-tasks. Furthermore, we propose two auxiliary losses corresponding to the two sub-tasks, to refine the representation learning in our model. Our extensive experiments not only demonstrate that the augmented representations in our model result in better performance than previous recommendation models, but also justify the impacts of the specially designed components in our model.

==> preliminary.tex <==
\section{Preliminary}
In this section, we first formalize the recommendation task addressed in this paper and then introduce the multi-task learning framework which is the basic framework of our group purchase recommendation model.

\subsection{Task Formalization}\label{sec:task}

%In the group buying process, a user will browse through all the items recommended on the platform. If the user finds an item interests him, he can buy this item at a better price by joining a group. There will be some groups already established the user can directly participate in. Of course, without suitable group, he can also set up a new group himself and wait for others to join it. A group purchase is divided into two steps toward success: the first step is a user to find an item of interest and initiate the group, and the second step is other users participate in the group continuously. Referring to [], we distinguish the identity of the user who initiates the group and the user who participates in the group, the former is called the initiator and the latter is called the participant.

At first, we use $u$, $i$, $p$ to represent an initiator, item and participant, respectively. According to our description about the group purchase process, the two sub-tasks of achieving group purchase recommendation can be formalized as: (1) recommending an $i$ for a given $u$, and (2) recommending a $p$ for a given pair $(u,i)$. A recommendation model of group purchase recommendation can achieve these two sub-tasks' objectives through computing two scoring functions, i.e., $S(i|u)$ and $S(p|u,i)$. As other recommendation models, the recommended objects ($i$ and $p$) are determined based on computing $S(i|u)$ and $S(p|u,i)$ for all candidate $i$s and candidate $p$s, respectively.

Then, we explain the rationality of computing $S(i|u)$ and $S(p|u,i)$ to achieve the task of group purchase recommendation. Formally, given a observed purchase group $<u, i, G>$ where $G=\{p_1, p_2, ..., p_{|G|}\}$ is the participant group, a group purchase recommendation model should maximize the probability of observing this purchase group, that is $P(u, i, p_1,p_2, ..., p_{|G|})$. In general, a participant is not familiar with each other in a participant group, indicating that each participant is independent to each other. Thus, we have
%\begin{equation}
$$
\begin{aligned}
P(u, i, p_1, p_2, ..., p_{|G|}) = P(p_1, p_2, ..., p_{|G|}|u, i)P(i|u)P(u) \\
P(u, i, p_1, p_2, ..., p_{|G|}) \propto P(p_1, p_2, ..., p_{|G|}|u, i) P(i|u)\\
P(p_1, p_2, ..., p_{|G|}|u, i) = P(p_1|u, i)P(p_2|u, i)...P(p_{|G|}|u, i).\\
\end{aligned}
$$
%\end{equation}
Accordingly, the probability $P(i|u)$ and $P(p|u, i)$ should be maximized through the model's computation, which just correspond to (are proportional to) $S(i|u)$ and $S(p|u,i)$, respectively. 

The training set of our model learning is collected from the observed purchase groups. Specifically, for the observed group $<u, i, G>$, $(u, i)$ is a positive sample of the first sub-task, namely task A. And $(u, i, p_1), (u, i, p_2), ..., (u, i, p_{|G|})$ are the positive samples of the second sub-task, namely task B. For both task A and task B, their negative samples are generated through negative sampling, of which the details will be introduced in the following experiment section.

In addition, we denote all user set and item set as $\mathcal{U}$ and $\mathcal{I}$, respectively. Obviously, $u, p\in\mathcal{U}$ and $i\in\mathcal{I}$. We further use $\mathcal{N}^+$ and $\mathcal{N}^-$ to denote the positive samples and negative samples of model training, respectively.

%Formulaically, We consider $U = \left\{ u_1, u_2, ..., u_{|U|} \right\}$ and $I = \left\{ i_1, i_2, ..., i_{|I|} \right\}$ to denote the user set and item set, respectively. We denote all interaction behavior records as $ B = \left\{ <u_1, i_1, p^{(1)}_1,...,p^{(1)}_{|p^{(1)}|}>,  <u_2, i_2, p^{(2)}_1,...,p^{(2)}_{|p^{(2)}|}>,... \right\} $, and each interaction record indicates that user $u_i$ initiated the group of product $i_i$, and  users $p^{(i)}_1, p^{(i)}_2,...p^{(i)}_{|p^{(i)}|}$ participated in the group. Therefore, the task objective is a score $S(u,i,p_1,p_2,...,p_{|p|})$ that represents the probability of completing a successful grouping. Due to the large and indefinite number of participants mentioned before, it is not reasonable and costly to model all participants directly. In most cases, the participants of a group are strangers to each other, and based on the assumption of mutual independence, the task goal can be represented as follows.

%Consequently, our model has two objectives $S(i|u)$ and $S(p|i,u)$, which means to recommend items that may be of interest to initiator, and to recommend other potential participants to the group with initiator and items already given.

%\subsection{Multi-task Learning (PLE)}
%\Red{......}

